Resource Cooperation in MEC and SDN based Vehicular Networks

Internet of Things (IoT) systems require highly scalable infrastructure to adaptively provide services to meet various performance requirements. Combining Software-Defined Networking (SDN) with Mobile Edge Cloud (MEC) technology brings more flexibility for IoT systems. We present a four-tier task processing architecture for MEC and vehicular networks, which includes processing tasks locally within a vehicle, on neighboring vehicles, on an edge cloud, and on a remote cloud. The flexible network connection is controlled by SDN. We propose a CPU resource allocation algorithm, called Partial Idle Resource Strategy (PIRS) with Vehicle to Vehicle (V2V) communications, based on Asymmetric Nash Bargaining Solution (ANBS) in Game Theory. PIRS encourages vehicles in the same location to cooperate by sharing part of their spare CPU resources. In our simulations, we adopt four applications running on the vehicles to generate workload. We compare the proposed algorithm with Non-Cooperation Strategy (NCS) and All Idle Resource Strategy (AIRS). In NCS, the vehicles execute tasks generated by the applications in their own On-Board Units (OBU), while in AIRS vehicles provide all their CPU resources to help other vehicles offloading requests. Our simulation results show that our PIRS strategy can execute more tasks on the V2V layer and lead to fewer number of task (and their length) to be offloaded to the cloud, reaching up to 28% improvement compared to NCS and up to 10% improvement compared to AIRS.

==> sections/Variable-name.tex <==
\section{variable name}
\label{sec:names}

task $TA_{V_{i},t}$   ===   task $K(L_{K},D_{K})$ 
execute time $Edl_{TA_{V_{i},t}}$ at local === execute time $d_{c}^{l}(K)$ 
delay local run $Edl_{TA_{V_{i},t}}$ ==  $d^{l}(K)$
delay e/cloud   $d^{e}(K)$ 
delay neighbour run      =====$d^{g}(K)$
 communication delay $d^{g}_{m}(K)$ between vehicles and
 computational delay $d^{g}_{c}(K)$.
 
 
 task length  $L_{V_{i},t}$ =====  $L_{K}$ 
capacity of the vehicle $C_{Vi,t}$ represent the idle CPU resource of vehicle $V_{i}$ at time $t$======  $C_{i}(t)$

neigbhour idle resource   ===  $C_{j}(t)$

neighbor set  $N = \left \{ N_{1}, N_{2} ...,N_{j}\right \}$


  task delay tolerance time  $d_{limit, TA_{V_{i}}}$====   $d_{limit, K}$


 we denoted the V2V communication data rate with $b_{V}$










 max vehicle  computation ability $C_{vmax}$ this is 2000 MI in this paper
 capacity of the vehicle $C_{Vi,t}$ represent the idle CPU resource of vehicle $V_{i}$ at time $t$
 task owner$V_{i}$
 local execute time $t_{V_{i}}$
 maximum delay tolerance$t_{Max}$
 
%  task $W_{N_{i}}^{t}$   this is the vehicle $N_{i}$ generates task at time $t$
 
 computational capacity of the vehicle $C_{V}$
 current idle CPU capacity  $C_{v_{i}, t}$
 
 task $TA_{V_{i},t}$   the task owner is $V_{i}$  generated at time $t$
  task length $L_{V_{i},t}$  the task owner is $V_{i}$  generated at time $t$
  task delay tolerance time  $d_{limit, TA_{V_{i}}}$
  local estimate delay $Edl_{TA_{V_{i},t}}$ 
  estimate the \ac{V2V} delay $Edc_{TA_{V_{i},t}}$
  
 neighbor  idle CPU resource $C_{NV_{j}}$
 neighbor vehicle $NV_{j}$

$p_{TA_{V_{i},t}}$  process vi at t task time

V2V bandwidth communication bandwidth is $B_{V2V}$.

Maximum tolerable delay of the task

take into account
 In this respect, the workload orchestration problem
should take into account the states of both computational and
networking resources at hand
 
